Convergence of Distributed Stochastic Variance Reduced Methods without Sampling Extra Data

Stochastic variance reduced methods have gained a lot of interest recently for empirical risk minimization due to its appealing run time complexity. When the data size is large and disjointly stored on different machines, it becomes imperative to distribute the implementation of such variance reduced methods. In this paper, we consider a general framework that directly distributes popular stochastic variance reduced methods in the master/slave model, by assigning outer loops to the parameter server, and inner loops to worker machines. This framework is natural and friendly to implement, but its theoretical convergence is not well understood. We obtain a comprehensive understanding of algorithmic convergence with respect to data homogeneity by measuring the smoothness of the discrepancy between the local and global loss functions. We establish the linear convergence of distributed versions of a family of stochastic variance reduced algorithms, including those using accelerated and recursive gradient updates, for minimizing strongly convex losses. Our theory captures how the convergence of distributed algorithms behaves as the number of machines and the size of local data vary. Furthermore, we show that when the data are less balanced, regularization can be used to ensure convergence at a slower rate. We also demonstrate that our analysis can be further extended to handle nonconvex loss functions.

==> outline_proof_arxiv.tex <==
\section{Proof Outline} \label{sec:outline}

In this section, we outline the convergence proofs of D-SVRG (Theorem~\ref{thm:dissvrgII}), D-RSVRG (Theorem~\ref{thm:rsvrg}), D-SARAH in the strongly convex (Theorem~\ref{thm:dissarah}) and nonconvex (Theorem~\ref{thm:dissarah_nonc}) settings, while leaving the details and the convergence proof of D-MiG (Theorem~\ref{thm:dismig}) to the appendix. Throughout this section, we simplify the notations $y_k^{t,s}$ and $v_k^{t,s}$ by dropping the $t$ superscript and the $k$ subscript, whenever the meaning is clear, since it is often sufficient to analyze the convergence of a specific worker $k$ during a single round.


\subsection{D-SVRG (Theorem~\ref{thm:dissvrgII})} \label{sec:proof_dsvrg}
We generalize the analysis of SVRG using the dissipativity theory in \cite{Hu2018} to the analysis of D-SVRG, which might be of independent interest. We start with a quick review of  dissipativity theory.
Consider the following linear time-invariant system
	\[
	\xi_{k+1}= A\xi_{k} + B w_k,
	\]
 	where $\xi_k \in \mbR^{n_\xi}$ is the state and $w_k \in \mbR^{n_w}$ is the input. Dissipativity theory characterizes how the inputs $w_j$, $j = 0,1,2,\ldots$ drive the internal energy stored in the states $\xi_j$, $j = 0,1,2,\ldots$ via an energy function $V:\mbR^{n_\xi}\mapsto \mbR_+$ and a supply rate $S:\mbR^{n_\xi}\times \mbR^{n_w}\mapsto \mbR$. The theory aims to build the following dissipation inequality:
	\begin{equation} \label{eq:dissipation_eq}
	V(\xi_{k+1}) \le \rho^2 V(\xi_{k}) + S(\xi_{k},w_{k}),
	\end{equation}
	where $\rho \in (0,1]$. The inequality indicates that at least a fraction $(1-\rho^2)$ of the internal energy will dissipate at every iteration. 
	
	With an energy function $V(\xi) = \xi^\top P \xi$ and supply rates 
	\begin{equation}\label{eq:supply_rates}
	S_j(\xi, w) = [\xi^\top, w^\top]  X_j  [\xi^\top, w^\top]^\top ,
	\end{equation} we have
	\begin{equation}\label{equ:dissip}
	V(\xi_{k+1}) \le \rho^2 V(\xi_k) + \sum_{j=1}^J \lambda_j S_j(\xi_k, w_k)
	\end{equation}
	as long as there exist a positive semidefinite matrix $P$ and non-negative scalars $\lambda_j$ such that
	\begin{equation}\label{equ:lmi}
	\begin{bmatrix}
	A^\top P A - \rho^2 P & A^\top P B \\
    	B^\top P A & B^\top P B \\
	\end{bmatrix}
	-\sum_{j=1}^J \lambda_j X_j \preceq 0.
	\end{equation}
	In fact, by left multiplying $[\xi_k^\top, w_k^\top]$ and right multiplying $[\xi_k^\top, w_k^\top]^\top$ to (\ref{equ:lmi}), we recover (\ref{equ:dissip}). We can capture properties of the objective function such as co-coercivity and strong-convexity with \eqref{equ:lmi} and characterize the optimality of $\xi_k$ by $V(\xi_k)$, thus wrapping the convergence proof as the existence of $\rho\in (0,1)$ satisfying \eqref{equ:lmi}, which can be viewed as a generalized eigenvalue optimization problem \cite{lessard2016analysis}.
	 
	 Setting $\xi^s = y^s - x^*$, we can write the local update of D-SVRG via the following linear time-invariant system \cite{Hu2018}:
	\begin{equation*}
	\xi^{s+1} = \xi^s - \eta\left[\nabla \ell_{z}\paren{\subx^s}-\nabla \ell_z\paren{\subx^0} + \nabla f\paren{\subx^0}\right],
	\end{equation*}
where $z$ is selected uniformly at random from local data points $\mathcal{M}_k$, or equivalently,
	\begin{equation}
	\xi^{s+1} = A\xi^s + Bw^s,
	\end{equation}
	with $A = I_d$, $B = \begin{bmatrix}
	-\eta I_d & -\eta I_d
	\end{bmatrix}$, and
	\begin{equation*}
		w^s = \begin{bmatrix}
            	\nabla \ell_z\paren{\subx^s} - \nabla \ell_z\paren{x^*} \\
            	\nabla \ell_z\paren{x^*}-\nabla \ell_z\paren{\subx^0} + \nabla f\paren{\subx^0}
	           \end{bmatrix}.
	\end{equation*}
	Here, $I_d$ is the identity matrix of dimension $d$. 
	
	Recall the supply rate in \eqref{eq:supply_rates}. Since $\xi^s \in \mbR^d$ and $w^s \in \mbR^{2d}$, we will write $X_j$ as $X_j = \bar{X}_j \otimes I_d$, where $\bar{X}_j\in \mbR^{3\times 3}$. Following \cite{Hu2018}, we consider the supply rates characterized by the following matrices:
		\begin{equation} \label{eq:supply_rates_optionII}
    		\bar{X}_1 = 
    		\begin{bmatrix}
    		0 & 0 & 0\\
    		0 & 1 & 0\\
    		0 & 0 & 0\\
    		\end{bmatrix},
    		\bar{X}_2 = 
    		\begin{bmatrix}
    		0 & 0 & 0\\
    		0 & 0 & 0\\
    		0 & 0 & 1\\
    		\end{bmatrix},
    		\bar{X}_3 = 
    		\begin{bmatrix}
    		0 & -1 & -1\\
    		-1 & 0 & 0\\
    		-1 & 0 & 0\\
    		\end{bmatrix}.
		\end{equation}

We have the following lemmas which are proved in Appendix \ref{proof:lem:svrgop2} and \ref{proof:thm:SVRG_op2_pre}, respectively.

	\begin{lemma}
		\label{lem:svrgop2}
		Suppose that Assumption \ref{assum:l_smooth}, \ref{assum:l_convex}, \ref{assum:f_sc} and \ref{assum:f_restricted} hold with $c_k\leq c$.
	For the supply rates defined in \eqref{eq:supply_rates_optionII}, we have 
		\begin{equation*}
		\begin{cases}
    		\ex{S_1} \le 2L\ex{f(\subx^s) - f^*} + 2cL\ex{\norm{\subx^s-x^*}^2};\\
    		\ex{S_2} \le 4L\ex{f(\subx^0) - f^*} + c(4L + 2c)\ex{\norm{\subx^0 - x^*}^2};\\ 
  \ex{S_3} \le -2\ex{f(\subx^s) - f^*} + 3c\ex{\norm{\subx^s - x^*}^2}+ c\ex{\norm{\subx^0 - x^*}^2}. 
		\end{cases}
		\end{equation*}
	\end{lemma}
	 
	\begin{lemma}
	    \label{lem:SVRG_op2_pre}
		Suppose that Assumption \ref{assum:l_smooth}, \ref{assum:l_convex}, \ref{assum:f_sc} and \ref{assum:f_restricted} hold with $c_k\leq c$. If there exist non-negative scalars $\lambda_j,\ j = 1, 2, 3$, such that 
		\begin{equation}\label{eq:svrg_inequality}
		\lambda_3 - L\lambda_1-(2L\lambda_1+3\lambda_3)c/\sigma > 0
		\end{equation} 
		and
		\begin{equation}
		\label{LMI:SVRG2}
		\begin{bmatrix}
		0 & \lambda_3 - \eta & \lambda_3 - \eta \\
		\lambda_3 - \eta & \eta^2 - \lambda_1 & \eta^2 \\
		\lambda_3 - \eta & \eta^2 & \eta^2 - \lambda_2
		\end{bmatrix}
		\preceq 0
		\end{equation}
		hold. Then D-SVRG satisfies  
		\begin{align}	\label{equ:svrg2}
		& \ex{f (\subx^+) - f^*}   \le \paren{\lambda_3 - L\lambda_1-(2L\lambda_1+3\lambda_3)c/\sigma}^{-1}\\
		&\;\cdot\left[\frac{1}{\sigma m}+\frac{c}{\sigma}\paren{ (4L+2c)\lambda_2 + \lambda_3}+ 2L\lambda_2\right] \ex{f(\subx^0) - f^*} ,\nonumber
		\end{align} 
		where the final output $\subx^+$ is selected from $y^1, \cdots, y^{m}$ uniformly at random.
	\end{lemma}
		
We can now prove Theorem~\ref{thm:dissvrgII}. Set $\lambda_1 = \lambda_2 = 2\eta^2$, and $\lambda_3 = \eta$. We have \eqref{eq:svrg_inequality} holds with the step size $\eta < \dfrac{\sigma - 3c}{L(2\sigma+4c)} $, and (\ref{LMI:SVRG2}) holds since
$$	\begin{bmatrix}
	0 & 0 & 0 \\
	0 & -\eta^2 & \eta^2 \\
	0 & \eta^2 & -\eta^2
	\end{bmatrix}
	\preceq 0. $$
   	Applying Lemma~\ref{lem:SVRG_op2_pre} with the above choice of parameters, \eqref{equ:svrg2} can be written as
	\begin{align*} 
		\ex{f (\subx^+) - f^*} \le & \Bigg( \dfrac{1/(\eta m) + c\paren{(8L+4c)\eta+1}+4L\eta}{\sigma(1-2L\eta )- c(4L\eta + 3) } \Bigg) \cdot\ex{f(\subx^0) - f^*}.
	\end{align*}
	
When $c < \sigma /4$, by choosing $\eta = (1-4c/\sigma)(40L)^{-1}$, $m = 160\kappa(1-4c/\sigma)^{-2}$, a convergence rate no more than $\nu:= 1-\frac{1}{2}\cdot\frac{\sigma-4c}{\sigma-3c}$ is obtained. Therefore, after line 8 of Alg.~\ref{alg:general}, we have for D-SVRG,
\begin{align*}
		    \ex{f(\tx^{t+1})-f^*} &\le \frac{1}{n}\sum_{k=1}^n \ex{f(y_k^{t+})-f^*} \le \paren{1-\dfrac{1}{2}\cdot\dfrac{\sigma-4c}{\sigma-3c}}\ex{f(\tx^t)-f^*}.
\end{align*}
To obtain an $\epsilon$-optimal solution in terms of function value, we need $\mathcal{O}(\xi^{-1}\log(1 / \epsilon))$ communication rounds, where $\zeta = 1 - 4c/\sigma$. Per round, the runtime complexity at each worker is $\mathcal{O}(N/n + m)=\mathcal{O}(N/n + \zeta^{-2}\kappa )$, where the first term corresponds to evaluating the batch gradient over the local data in parallel, and the second term corresponds to evaluating the stochastic gradients in the inner loop. Multiplying this with the communication rounds leads to the overall runtime.

%Note that in the distributed setting, calculating the full-batch gradient only needs $\mathcal{O}(N/n)$ time instead of $\mathcal{O}(N)$ time due to parallelized computation, so the overall time complexity to find an $\epsilon$-optimal solution is
%		\[
%		\mathcal{O}\paren{(N/n + \zeta^{-2}\kappa)\zeta^{-1}\log(1/\epsilon)},
%		\] 


\subsection{D-RSVRG (Theorem~\ref{thm:rsvrg})}
\label{proof:rsvrg}

 
Consider an auxiliary sample function at the \sout{$t$th}{\color{red}$\tth{t}$} round and the \sout{$k$th}{\color{red}$\tth{k}$} worker as
\[
\ell_{\mu_k}^t(x;z) = \ell(x;z) + \frac{\mu_k}{2}\norm{x - \tx^t}^2.
\]
This leads to the auxiliary local and global loss functions, respectively,
\[
f^t_i(x) = \frac{1}{|\mathcal{M}_i|}\sum_{z\in \mathcal{M}_i}\ell^t_{\mu_k}(x;z) = f_i(x) + \frac{\mu_k}{2}\norm{x - \tx^t}^2,  
\]
for $1\leq i \leq n$, and
\begin{equation}\label{eq:auxiliary_loss}
f^t(x) = \frac{1}{n}\sum_{i=1}^n f^t_i(x) = f(x) + \frac{\mu_k}{2}\norm{x - \tx^t}^2.
\end{equation}
Moreover, we have 
\begin{align*}
& \quad \nabla \ell_{\mu_k}^t(\subx_{k}^{t,s+1};z) -\nabla \ell_{\mu_k}^t(\tx^{t};z) + \nabla f^t(\tx^{t})\\
&=\nabla \ell(\subx_{k}^{t,s+1};z) -\nabla \ell(\tx^{t};z) + \nabla f(\tx^{t}) + \mu_k (\subx_{k}^{t,s+1} - \tx^t),
\end{align*}
which means that D-RSVRG performs in exactly the same way as the unregularized D-SVRG with the auxiliary loss functions $\ell_{\mu_k}^t$ in the \sout{$t$th}{\color{red}$\tth{t}$} round. Note that $\ell_{\mu_k}^t$ is $(\mu_k + L)$-smooth and that $f^t$ is $(\mu_k + \sigma)$-strongly-convex, while the restricted smoothness of the \sout{$k$th}{\color{red}$\tth{k}$} worker, $f^t - f_k^t = f - f_k$ remains unchanged. Applying Theorem~\ref{thm:dissvrgII}, we have 
 \begin{equation}\label{eq:auxiliary_descent}
\ex{f^t(\tx^{t+1}) - f^{t*}} < \nu \ex{f^t(\tx^t) - f^{t*}},
\end{equation}
where $f^{t*}$ is the optimal value of $f^t$, when Assumptions \ref{assum:l_smooth}, \ref{assum:l_convex} and \ref{assum:f_sc} hold, and Assumption~\ref{assum:f_restricted} holds, as long as $c_k < (\sigma+\mu_k)/4$, along with proper $m$ and step size $\eta$.


However, the definition of the regularized loss functions $\ell^t_{\mu}$ and ${f}^t$ rely on $\tx^t$, which changes over different rounds. Our next step is to relate the descent of $f^t$ to $f$. To this end, we have
\begin{align*}
& \ex{f(\tx^{t+1}) - f^*} \\
=& \ex{f^t(\tx^{t+1}) - f^{t*}} + f^{t*} - \ex{\frac{\mu}{2}\norm{\tx^t - \tx^{t+1}}^2} - f^* \\
<& \ex{ f^t(\tx^t) - f^{t*} } - (1-\nu)\ex{f^t(\tx^t) - f^{t*}} + f^{t*} - f^* \\
=& \ex{f(\tx^t) - f^*} - (1-\nu)\ex{f(\tx^t) - f^{t*} },
\end{align*}
where the second line uses \eqref{eq:auxiliary_loss}, the third line uses \eqref{eq:auxiliary_descent}, and the last line follows from $f(\tx^t) = f^t(\tx^t)$.

We can continue to bound $f(\tx^t) - f^{t*}$ in two manners. First, $f(\tx^t) - f^{t*} = f^t(\tx^t) - f^{t*} > \frac{1}{2(L+\mu)}\norm{\nabla f (\tx^t)}^2 > \frac{\sigma}{L+\mu}(f(\tx^t) - f^*)$. 
On the other hand, we have $f(\tx^t) -f^{t*} \ge f(\tx^t) - f^t(x^*) = f(\tx^t) - f(x^*) - \frac{\mu}{2}\norm{\tx^t - x^*}^2 \ge (1-\mu/\sigma)(f(\tx^t) - f^*)$. Thus \eqref{eq:rate_drsvrg} follows immediately by combining the above two bounds.
 
 

\subsection{D-SARAH in the Strongly Convex Case (Theorem~\ref{thm:dissarah})}

 Theorem~\ref{thm:dissarah} can be deducted from the following theorem, whose proof can be found in Appendix \ref{proof:thm:SARAH_pre}.
\begin{theorem}
    \label{thm:SARAH_pre}
	Suppose that Assumption \ref{assum:l_smooth}, \ref{assum:l_convex}, \ref{assum:f_sc} and \ref{assum:f_restricted} hold with $c_k\leq c$.
	 Then D-SARAH satisfies
	\begin{align*}
		     \paren{1-\frac{4c^2}{\sigma^2}} & \ex{\norm{\nabla f(\tx^{t+1})}^2} \le\paren{\frac{1}{\sigma\eta m} + \frac{4c^2}{\sigma^2}+\frac{2\eta L}{2-\eta L}}\ex{\norm{\nabla f(\tx^t)}^2}.
	\end{align*}
\end{theorem}
When $c < \frac{\sqrt{2}}{4} \sigma$, we can choose $\eta = \dfrac{2(1-8c^2/\sigma^2)}{(9-8c^2/\sigma^2)L}$ and $m = 2\kappa\dfrac{9-8c^2/\sigma^2}{(1-8c^2/\sigma^2)^2}$ in Theorem~\ref{thm:SARAH_pre}, leading to the following convergence rate:
	\[
\ex{\norm{\nabla f(\tx^{t+1})}^2}\\
		\le\frac{1}{2-8c^2/\sigma^2}\ex{\norm{\nabla f(\tx^t)}^2}.
	\]
    Consequently, following similar discussions as D-SVRG, the communication complexity of finding an $\epsilon$-optimal solution is $\mathcal{O}(\zeta^{-1}\log(1/\epsilon))$, and the runtime complexity is
$    \mathcal{O}\paren{(N/n + \zeta^{-2}\kappa)\zeta^{-1}\log(1/\epsilon)}$,    where $\zeta = 1 - 2\sqrt{2}c/\sigma$.


\subsection{D-SARAH in the Nonconvex Case (Theorem \ref{thm:dissarah_nonc})}

Theorem \ref{thm:dissarah_nonc} can be deducted from the following theorem, proved in Appendix~\ref{proof:thm:SARAH_nonc}, which specifies the choice of the step size to guarantee convergence.

\begin{theorem}
    \label{thm:SARAH_nonc}
    Suppose that Assumption \ref{assum:l_smooth} and \ref{assum:f_nrestricted} hold with $c_k\leq c$. By setting the step size
    \[
    \eta \le \frac{2}{L\paren{1+\sqrt{1+8(m-1)+4m(m-1)c^2/L^2}}},
    \]
     For a single outer loop of D-SARAH, it satisfies:
    \[
    	\sum_{s=0}^{m-1} \ex{\norm{\nabla f(y^s)}^2} \le \frac{2}{\eta} \ex{f(y^0) - f(y^{m})}.
    \]
\end{theorem}

By setting $\tx^{t+1} = y^{m}$, from the above theorem, we have 
\[
\sum_{s=0}^{m-1} \ex{\norm{\nabla f(y^s)}^2} \le \frac{2}{\eta} \ex{f(\tx^t) - f(\tx^{t+1})}.
\]
Hence, with $T$ outer loops, we have
\[
\frac{1}{Tm}\sum_{t=0}^{T-1}\sum_{s=0}^{m-1} \ex{\norm{\nabla f(y^{t,s}_{k(t)})}^2} \le\frac{2}{\eta Tm}\paren{f(\tx^0) - f^*}.
\]
where  $k(t)$ is the worker index selected in the \sout{$t$th}{\color{red}$\tth{t}$} round for parameter update.
The communication complexity to achieve an $\epsilon$-optimal solution is
\begin{align*}
T =& \mathcal{O}\paren{1+ \frac{1}{\eta m \epsilon}} = \mathcal{O}\paren{1+\frac{\sqrt{m+m^2c^2/L^2}}{m}\cdot\frac{L}{\epsilon}} \\
=& \mathcal{O}\paren{1+\paren{\frac{1}{\sqrt{m}}+\frac{c}{L}}\cdot \frac{L}{\epsilon}},
\end{align*}
with the choice $\eta = \Theta\paren{\frac{1}{L\sqrt{m+m^2c^2/L^2}}}$. Per round, the runtime complexity at each worker is $\mathcal{O}(N/n + m)$. By choosing $m = \mathcal{O}(N/n)$,
we achieve the runtime complexity 
$$\tiny \mathcal{O}\paren{N/n + \paren{\sqrt{N/n} + N/n\cdot \frac{c}{L}}\frac{L}{\epsilon}}.$$
 


==> proof_outline_dmig.tex <==


\subsection{Proof of Theorem~\ref{thm:dismig}} \label{sec:proof_dmig}
\yc{let's move Proof of Theorem~\ref{thm:dismig} back to the supplemental materials - in single column format (use the arxiv version?)}
As earlier, we simplify the notations $y_k^{t,s}$, $x_k^{t,s}$ and $v_k^{t,s}$ by dropping the  superscript $t$ and the  subscript $k$. In this section we deal with the non-smooth target function $F(x) = f(x) + g(x)$ as mentioned in Remark~\ref{remark:dig}, where $g$ is a convex and non-smooth function known to all agents. The analysis is done by carefully adapting the proof for the centralized algorithm (i.e. \cite[Section B.1.]{zhou2018simple}) with the distributed smoothness assumption. 
We impose the following constraint on the step size $\eta$:
\begin{equation}\label{eq:stepsize_constraint}
	L\theta + \frac{L\theta}{1-\theta} + c \le \frac{1}{\eta}.
\end{equation}
From \cite[Equations (8) and (9)]{zhou2018simple}, we have
\begin{align}
	f(y^{s-1}) - f(u) &\le \frac{1-\theta}{\theta}\innprod{\nabla f(y^{s-1}), \tx - y^{s-1}} \nonumber \\
	&\qquad + \innprod{\nabla f(y^{s-1}), x^{s-1}-u}, 	\label{eq:MiG_1} \\
	\innprod{\nabla f(y^{s-1}), x^{s-1}-u}&  = \innprod{\nabla f(y^{s-1}) - \tilde{\nabla}, x^{s-1}-u}\nonumber \\
	& \hspace{-0.3in}   + \innprod{\tilde{\nabla}, x^{s-1}-x^s} + \innprod{\tilde{\nabla}, x^{s}-u},
	\label{eq:MiG_2}
\end{align}
where $\tilde{\nabla} = \nabla\ell_z(y^{s-1})-\nabla\ell_z(\tx)+\nabla f(\tx)$, with $z$ randomly selected from $\mathcal{M}_k$ and $u\in \mbR^d$ is an arbitrary vector. Following the $L$-smoothness argument in \cite{zhou2018simple}, \eqref{eq:MiG_2} leads to
\begin{align*}
	&\innprod{\tilde{\nabla}, x^{s-1}-x^s}  \le \frac{1}{\theta}\paren{f(y^{s-1})-f(y^s)} \nonumber \\
	&\quad +\innprod{\nabla f(y^{s-1})-\tilde{\nabla}, x^{s}-x^{s-1}} + \frac{L\theta}{2}\norm{x^{s}-x^{s-1}}^2 .
\end{align*}
By plugging in the constraint \eqref{eq:stepsize_constraint}, we have
\begin{align}
&\innprod{\tilde{\nabla},  x^{s-1}-x^s} \le  \frac{1}{\theta}\paren{f(y^{s-1})-f(y^s)} \notag \\
&\qquad+\innprod{x^{s}-x^{s-1}} \notag \\
& \qquad + \paren{\frac{1}{2\eta}-\frac{L\theta}{2(1-\theta)}-\frac{c}{2}}\norm{x^{s}-x^{s-1}}^2.
\label{eq:MiG_3}
\end{align}
By combining \eqref{eq:MiG_1},\eqref{eq:MiG_2},\eqref{eq:MiG_3}, \cite[Lemma 3]{zhou2018simple} and then taking expectation over the choice of random sample $z$, we have
\begin{equation}
	\begin{aligned}
		& f(y^{s-1}) - f(u) \\
		\le& \frac{1-\theta}{\theta}\innprod{\nabla f(y^{s-1}), \tx - y^{s-1}} + \ex{\innprod{\nabla f(y^{s-1}) - \tilde{\nabla},x^{s} - u}} \\
		& + \frac{1}{\theta}\paren{f(y^{s-1}) - \ex{f(y^s)}} -\paren{\frac{L\theta}{2(1-\theta)}+\frac{c}{2}}\ex{\norm{x^s - x^{s-1}}^2} \\
		&+ \frac{1}{2\eta} \norm{x^{s-1}-u}^2 - \frac{1+\eta \sigma}{2\eta}\ex{\norm{x^s - u}^2} + g(u) - \ex{g(x^s)}.
	\end{aligned}
	\label{equ:mig_ref}
\end{equation}
%Note that the additional $\frac{c}{2}\norm{x^s-x^{s-1}}^2$ term is due to $c$'s presence in our version of constraint.
We further split the term $\ex{\innprod{\nabla f(y^{s-1}) - \tilde{\nabla},x^{s} - u}}$ as
\begin{align*}
& \ex{\innprod{\nabla f(y^{s-1}) - \tilde{\nabla},x^{s} - u}} \\
=&\ex{\innprod{\nabla f(\tx) - \nabla f_k(\tx) +\nabla f_k(y^{s-1}) - \tilde{\nabla},x^{s} - x^{s-1}}} \\
&   +\ex{\innprod{\nabla f(y^{s-1}) - \tilde{\nabla},x^{s-1} - u}}\\
&+\ex{\innprod{\nabla f(y^{s-1})-\nabla f(\tx) + \nabla f_k(\tx) -\nabla f_k(y^{s-1}),x^{s} - x^{s-1}}} \\
\le&\frac{1}{2\beta}\ex{\norm{\nabla f(\tx) - \nabla f_k(\tx) +\nabla f_k(y^{s-1}) - \tilde{\nabla}}^2} \\
& + \frac{\beta}{2}\ex{\norm{x^{s} - x^{s-1}}^2}+c\norm{\tx - y^{s-1}}\ex{\norm{x^s - x^{s-1}}} \\
&+ c\norm{\tilde{x}-y^{s-1}}\norm{x^{s-1}-u}\\
\le&\frac{1}{2\beta}\paren{2LD_f(\tx, y^{s-1})+2cL\norm{\tx-y^{s-1}}^2} \\
& + \frac{\beta + c}{2}\ex{\norm{x^{s} - x^{s-1}}^2} +c\norm{\tx - y^{s-1}}^2  + \frac{c}{2}\norm{x^{s-1}-u}^2,
\end{align*}
where the first inequality is due to Cauchy-Schwarz inequality and Assumption \ref{assum:f_nrestricted}, with $\beta > 0$ satisfying $\frac{1-\theta}{\theta} = \frac{L}{\beta}$, and the last inequality is obtained by combining
\small
\[
\ex{\norm{\nabla f(\tx) - \nabla f_k(\tx) +\nabla f_k(y) - \tilde{\nabla}}^2} \le \ex{\norm{\nabla \ell_z(y^{s-1})-\nabla \ell_z(\tx)}^2}.
\]
\normalsize
with Lemma~\ref{lem:rsp666} under Assumption~\ref{assum:f_nrestricted}, along with the inequality $ab \le (a^2+b^2)/2$. By substituting the inequality into (\ref{equ:mig_ref}) we have the following result:
\begin{align*}
&  f(y^{s-1}) - f(u) \\
 \le& \frac{1}{2\beta}\ex{2L(f(\tx)-f( y^{s-1})+2cL\norm{\tx-y^{s-1}}^2} \\
 & +c\norm{\tx - y^{s-1}}^2 + \frac{c}{2}\norm{x^{s-1}-u}^2 + \frac{1}{\theta}\paren{f(y^{s-1}) - \ex{f(y^s)}}\\
& + \frac{1}{2\eta} \norm{x^{s-1}-u}^2 - \frac{1+\eta \sigma}{2\eta}\ex{\norm{x^s - u}^2} + g(u) - \ex{g(x^s)}\\
\le& c\theta\norm{\tx-x^{s-1}}^2 + \frac{c}{2}\norm{x^{s-1}-u}^2 \\
& + \frac{1-\theta}{\theta}\paren{f(\tx)-f( y^{s-1})} + \frac{1}{\theta}\paren{f(y^{s-1}) - \ex{f(y^s)}} \\
& + \frac{1}{2\eta} \norm{x^{s-1}-u}^2 - \frac{1+\eta \sigma}{2\eta}\ex{\norm{x^s - u}^2} + g(u) - \ex{g(x^s)}.
\end{align*}
Note that the choice of $\beta$ cancels $\frac{1-\theta}{\theta}\innprod{\nabla f(y^{s-1}), \tx - y^{s-1}}$ and $\paren{\frac{L\theta}{2(1-\theta)}+\frac{c}{2}}\ex{\norm{x^s - x^{s-1}}^2}$. By rearranging the above inequality, we can cancel the term $f(y^{s-1})$. We further use $-g(x^s)\le\frac{1-\theta}{\theta}g(\tx) - \frac{1}{\theta}g(y^s)$, which leads to 
\[
\begin{aligned}
&\frac{1}{\theta}\paren{\ex{F(y^s)} - F(u)} \le c\theta\norm{\tx-x^{s-1}}^2 + \frac{1-\theta}{\theta}\paren{F(\tx)-F(u)} \\
&\quad+ \frac{1+c\eta}{2\eta} \norm{x^{s-1}-u}^2 - \frac{1+\eta \sigma}{2\eta}\ex{\norm{x^s - u}^2}.
\end{aligned}
\]
Note that $\norm{\tx - x^{s-1}}^2 \le 2\norm{\tx - x^*}^2 + 2\norm{x^{s-1}-x^*}^2$. By setting $u = x^*$
and using $\sigma$-strongly-convexity of $F$ we have
\[
\begin{aligned}
& \frac{1}{\theta}\paren{\ex{F(y^s)} - F^*}\le \paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}\paren{F(\tx)-F^*} \\
&\; + \frac{1+(1+4\theta)c\eta}{2\eta} \norm{x^{s-1}-x^*}^2 - \frac{1+\eta \sigma}{2\eta}\ex{\norm{x^s - x^*}^2}.
\end{aligned}
\]
To simplify the analysis we impose another constraint $\theta \le 1/2$:
\begin{equation}
\begin{aligned}
&\frac{1}{\theta}\paren{\ex{F(y^s)} - F^*}\le \paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}\paren{F(\tx)-F^*} \\
&   + \frac{1+3c\eta}{2\eta} \norm{x^{s-1}-x^*}^2 - \frac{1+\eta \sigma}{2\eta}\ex{\norm{x^s - x^*}^2}.
\end{aligned}
\label{equ:mig_onestep}
\end{equation}
Let $w = \frac{1+\eta\sigma}{1+3c\eta}$. Multiplying (\ref{equ:mig_onestep}) by $w^{s-1}$ and then summing over $s$, we have
\small
\[
\begin{aligned}
&\frac{1}{\theta}\sum_{s=0}^{m-1} w^s(\ex{F(y^{s+1})}-F^*) + \frac{w^m(1+3c\eta)}{2\eta}\ex{\norm{x^m - x^*}^2} \\
\le& \paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}\sum_{s=0}^{m-1} w^s(F(\tx)-F^*)+\frac{1+3c\eta}{2\eta}\norm{x^0 - x^*}^2,\\
\end{aligned}
\]
\normalsize
Adding the superscript $t$ and the subscript $k$ back and applying Jensen's inequality to the definition of $y_k^{t+}$, we get
\small
\[
\begin{aligned}
&\frac{1}{\theta}\sum_{s=0}^{m-1} w^s(\ex{F(y_k^{t+})}-F^*) + \frac{w^m(1+3c\eta)}{2\eta}\ex{\norm{x^{t+1,0}_k - x^*}^2} \\
\le& \paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}\sum_{s=0}^{m-1} w^s(F(\tx^t)-F^*)+\frac{1+3c\eta}{2\eta}\norm{x^{t,0}_k - x^*}^2.
\end{aligned}
\]
\normalsize
Averaging the inequality over $k = 1,\cdots, n$, we have
\small
\[
\begin{aligned}
&\frac{1}{\theta}\sum_{s=0}^{m-1} w^s(\ex{F(\tx^{t+1})}-F^*) \\
& \quad+ \frac{w^m(1+3c\eta)}{2\eta}\ex{\frac{1}{n}\sum_{k=1}^n\norm{x^{t+1,0}_k - x^*}^2} \\
\le& \paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}\sum_{s=0}^{m-1} w^s(F(\tx^t)-F^*) \\
& \quad +\frac{1+3c\eta}{2\eta}\frac{1}{n}\sum_{k=1}^n\norm{x^{t,0}_k - x^*}^2.
\end{aligned}
\] 
\normalsize

\paragraph{Case I}
$\frac{m(\sigma-3c)}{L} \le 3/4$. By setting $\theta = \sqrt{\frac{m(\sigma-3c)}{3L}} \le 1/2$ and $\eta = \frac{1}{3L\theta+c}$ we satisfy the step size constraint \eqref{eq:stepsize_constraint}. We aim to show that
\[
\frac{1}{\theta} \ge \paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}w^m.
\]
We have $w = \frac{1+\eta\sigma}{1+3c\eta} \le 1 + \eta \sigma - 3c\eta$. Note that $L\theta = \sqrt{\frac{Lm(\sigma-3c)}{3}} \ge \sqrt{\frac{\sigma(\sigma-3c)}{3}} >c$, so $\eta \le \frac{1}{4L\theta}$. Moreover, with $\sigma > 8c$ we have  
\[
\frac{\frac{m}{4L\theta}(\sigma-3c)}{\theta-\frac{4c}{\sigma}\theta^2} = \frac{3}{4(1-4c\theta/\sigma)} \le 1.
\]
Hence,
\begin{align*}
& \paren{1-\theta+\frac{4c}{\sigma}\theta^2}\paren{1+\eta\sigma-3\eta c}^m \\
& \le \paren{1-\theta+\frac{4c}{\sigma}\theta^2}\paren{1+\frac{1}{4L\theta}(\sigma - 3c)}^m \\
&\le \paren{1-\zeta}\paren{1+\zeta/m}^m,
\end{align*}
where $\zeta =\frac{m}{4L\theta}(\sigma - 3c)$. With $\zeta \le \theta - \frac{4c}{\sigma}\theta^2 \le 1/2$ we have $\paren{1-\zeta}\paren{1+\zeta/m}^m \le 1$. So we have
\small
\begin{align*}
\paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}w^m & \ge \frac{1}{\theta}\paren{1-\theta+\frac{4c}{\sigma}\theta^2}\paren{1+\eta\sigma-3\eta c}^m   \ge \frac{1}{\theta}.
\end{align*}
\normalsize

Therefore we have
\small
\[
\begin{aligned}
&w^m\bigg(\paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}\sum_{s=0}^{m-1} w^s(F(\tx^{t+1})-F^*)  \\
& \quad + \frac{1+3c\eta}{2\eta}\ex{\frac{1}{n}\sum_{k=1}^n\norm{x^{t+1,0}_k - x^*}^2}\bigg) \\
\le& \paren{\frac{1-\theta}{\theta}+\frac{4c\theta}{\sigma}}\sum_{s=0}^{m-1} w^s(F(\tx^t)-F^*) \\
& +\frac{1+3c\eta}{2\eta}\frac{1}{n}\sum_{k=1}^n\norm{x^{t,0}_k - x^*}^2.
\end{aligned}
\]
\normalsize
The convergence rate over $T$ rounds of communication is $w^{-Tm} = \paren{1+\Theta\paren{\frac{1}{\sqrt{3\kappa m}}}}^{-Tm}$, so the communication complexity is $T=\mathcal{O}\paren{\sqrt{\kappa/m}\log(1/\epsilon)}$. With the choice of $m = \Theta(N/n)$ the runtime complexity is $\mathcal{O}((N/n+m)T)=\mathcal{O}(\sqrt{\kappa N/n}\log(1/\epsilon))$.


\paragraph{Case II}
$\frac{m(\sigma-3c)}{L} > 3/4$. We set $\theta = 1/2$ and $\eta = \frac{1}{3L\theta+c}$.
We have $\eta\sigma = \frac{1}{3\kappa/2 + c/\sigma} \le 2/3$, thus 
\[
w = \frac{1+\eta\sigma}{1+3c\eta} \ge \frac{1+2/3+\eta\sigma-3c\eta}{1+2/3} = 1 + \frac{3}{5}\paren{\eta \sigma - 3c\eta}
\]
and $w^m \ge 1+\frac{3}{5}(\sigma-3c)\eta m	\ge 1+\frac{3m(\sigma-3c)}{5(3L/2+L/8)}>1+1/4$. So we have
\small
\[
\begin{aligned}
&2\sum_{s=0}^{m-1} w^s(F(\tx^{t+1})-F^*) \\
&\quad + \frac{5}{4}\cdot\frac{1+3c\eta}{2\eta}\ex{\frac{1}{n}\sum_{k=1}^n\norm{x^{t+1,0}_k - x^*}^2} \\
\le& \paren{1+\frac{1}{4}}\sum_{s=0}^{m-1} w^s(F(\tx^t)-F^*)+\frac{1+3c\eta}{2\eta}\frac{1}{n}\sum_{k=1}^n\norm{x^{t,0}_k - x^*}^2.
\end{aligned}
\]
\normalsize
Therefore,
\small
\[
\begin{aligned}
&\frac{5}{4}\bigg( \frac{5}{4}\sum_{s=0}^{m-1} w^s(F(\tx^{t+1})-F^*)  \\
& \quad + \frac{1+3c\eta}{2\eta}\ex{\frac{1}{n}\sum_{k=1}^n\norm{x^{t+1,0}_k - x^*}^2} \bigg)  \\
\le& \frac{5}{4}\sum_{s=0}^{m-1} w^s(F(\tx^t)-F^*)+\frac{1+3c\eta}{2\eta}\frac{1}{n}\sum_{k=1}^n\norm{x^{t,0}_k - x^*}^2.
\end{aligned}
\]
\normalsize
This implies that $\mathcal{O}(\log(1/\epsilon))$ rounds of communication is sufficient to find an $\epsilon$-accurate solution, and that the runtime complexity is $\mathcal{O}(N/n\log(1/\epsilon))$.


==> proof_outline_dsarah.tex <==


\section{Proof for D-SARAH} \label{sec:proof_dsarah}

    
    
\subsection{Proof of Theorem \ref{thm:SARAH_pre}}
\label{proof:thm:SARAH_pre}


To begin, we cite   a supporting lemma from \cite{Nguyen2017}.

\begin{lemma}\cite{Nguyen2017}
	\label{lem:v_concaten}
	Suppose Assumption \ref{assum:l_smooth} and \ref{assum:l_convex} hold and $\eta < 2/L$, then 	
	\[
		\ex{\norm{v^s - v^{s-1}}^2} \le \frac{\eta L}{2-\eta L} \left[ \ex{\norm{v^{s-1}}^2}  - \ex{\norm{v^s}^2} \right].
	\] 
\end{lemma}
 

We also present a new lemma below with the proof given in Appendix \ref{proof:lem:trace_concaten}.
\begin{lemma}
	\label{lem:trace_concaten}
	The update rule of D-SARAH satisfies
\begin{align*}
			&\ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s) - v^s}^2} \\ =& \sum_{j=1}^s \ex{\norm{v^j-v^{j-1}}^2} \\
			&\quad- \sum_{j=1}^s\ex{\norm{\nabla f_k(y^j) - \nabla f_k(y^{j-1})}^2}.
		\end{align*}
\end{lemma}

\begin{proof}[Proof of Theorem \ref{thm:SARAH_pre}]
By combining Lemmas \ref{lem:v_concaten} and \ref{lem:trace_concaten}, we have
\begin{align}\label{eq:term1}
& \ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s) - v^s}^2} \nonumber\\
\le& \sum_{j=1}^s \ex{\norm{v^j-v^{j-1}}^2}  \le  \frac{\eta L}{2-\eta L}\ex{\norm{v^0}^2}.
\end{align}
By Assumption \ref{assum:f_restricted}, we have
\begin{align}\label{eq:term2}
	&\quad \norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s)   - \nabla f(y^s)  }^2\nonumber \\
	&= \norm{\nabla (f-f_k)(y^0) - \nabla (f-f_k)(y^s)}^2\nonumber\\
	&\le 2c^2\norm{y^s-x^*}^2+2c^2\norm{y^0-x^*}^2.
\end{align}
Therefore, combining \eqref{eq:term1} and \eqref{eq:term2}, we have
\begin{align*}
& \ex{\norm{\nabla f(y^s) - v^s}^2} \\
\le& 2 \ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s)   - \nabla f(y^s)  }^2}\\
&\quad+2\ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s) - v^s}^2}\\
\le&  4c^2\ex{\norm{y^s-x^*}^2}+4c^2\ex{\norm{y^0-x^*}^2} \\
&\quad+ \frac{2\eta L}{2-\eta L}\ex{\norm{v^0}^2} .
\end{align*}
Substituting it into Lemma \ref{lem:grad_comp} gives 
\[
\begin{aligned}
	&\sum_{s=0}^{m-1} \ex{\norm{\nabla f(y^s)}^2} \\
		\le& \frac{2}{\eta} \ex{f(y^0) - f(x^*)} + \sum_{s=0}^{m-1} \ex{\norm{\nabla f(y^s) - v^s}^2} \\
	\le& \frac{2}{\eta} \ex{f(y^0 )- f(x^*)} +\sum_{s=0}^{m-1} \Big(4c^2\ex{\norm{y^s-x^*}^2} \\
	&\quad+4c^2\ex{\norm{y^0-x^*}^2} + \frac{2\eta L}{2-\eta L}\ex{\norm{v^0}^2} \Big) .
\end{aligned}
\]
Since $f$ is $\sigma$-strongly convex, we have $4c^2\norm{y^s-x^*}^2 \le \frac{4c^2}{\sigma^2}\norm{\nabla f(y^s)}^2$. Denote $y^+$ as the local update which is selected from $y^0, \cdots, y^{m-1}$ uniformly at random. We have
\[
\begin{aligned}	
	& \paren{1-\frac{4c^2}{\sigma^2}}\ex{\norm{\nabla f(y^+)}^2} \\
	=& \paren{1-\frac{4c^2}{\sigma^2}}\frac{1}{m}\sum_{s=0}^{m-1} \ex{\norm{\nabla f(y^s)}^2} \\
	\le& \frac{2}{\eta m} \ex{f(y^0) - f(x^*)} + 4c^2\ex{\norm{y^0-x^*}^2} \\
	& \quad\quad\quad + \frac{2\eta L}{2-\eta L}\ex{\norm{v^0}^2} \\
	\le& \paren{\frac{1}{\sigma\eta m} + \frac{4c^2}{\sigma^2}+\frac{2\eta L}{2-\eta L}}\ex{\norm{\nabla f(y^0)}^2}.
\end{aligned}
\]
Since $\tx^{t+1}$ is randomly chosen from the local outputs $\{y_k^{t+},\ 1\le k \le n\}$, we have
\begin{align*}
& \paren{1-\frac{4c^2}{\sigma^2}}\ex{\norm{\nabla f(\tx^{t+1})}^2} \\
& \quad \le\paren{\frac{1}{\sigma\eta m} + \frac{4c^2}{\sigma^2}+\frac{2\eta L}{2-\eta L}}\ex{\norm{\nabla f(\tx^t)}^2}.
\end{align*}
 \end{proof}



\subsection{Proof of Theorem~\ref{thm:SARAH_nonc}}\label{proof:thm:SARAH_nonc}
   
Recall Lemma \ref{lem:grad_comp}. The theorem follows if  
	$$\sum_{s=0}^{m-1} \ex{\norm{\nabla f(y^s) - v^s}^2} - (1-L\eta)\sum_{s=0}^{m-1}\ex{\norm{v^s}^2} \leq 0 . $$ 
The rest of this proof is thus dedicated to show the above inequality. 

Note that
    \begin{align*}
    &\ex{\norm{\nabla f(y^s) - v^s}^2} \\
    \le& 2 \ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s) -  \nabla f(y^s) }^2}\\
    &\quad+2\ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s) - v^s}^2}\\
    \le& 2c^2 \ex{\norm{y^0 - y^s}^2} + 2\sum_{j=1}^s \ex{\norm{v^j-v^{j-1}}^2}\\
    \le& 2c^2s\sum_{j=1}^s \ex{\norm{y^j-y^{j-1}}^2} + 2\sum_{j=1}^s \ex{\norm{v^j-v^{j-1}}^2}\\
    =& 2c^2s\eta^2 \sum_{j=1}^s \ex{\norm{v^{j-1}}^2} + 2\sum_{j=1}^s \ex{\norm{v^j-v^{j-1}}^2},
    \end{align*}
    where the second inequality follows from Lemma~\ref{lem:trace_concaten} and Assumption~\ref{assum:f_nrestricted}, and the third inequality follows from $y^0-y^s = \sum_{j=1}^s y^j -y^{j-1}$, and the last line follows from the definition. The $L$-smoothness of $ \ell_z$ implies that
    \begin{align*}
    	\norm{v^j-v^{j-1}}^2 &= \norm{\nabla \ell_z\paren{y^j}-\nabla \ell_z\paren{y^{j-1}}}^2 \\
	& \le L^2\norm{y^j-j^{j-1}}^2 = L^2\eta^2 \norm{v^{j-1}}^2.
    \end{align*}
    So we have
    \begin{align*}
	    &\sum_{s=0}^{m-1} \ex{\norm{\nabla f(y^s) - v^s}^2} - (1-L\eta)\sum_{s=0}^{m-1}\ex{\norm{v^s}^2} \\
	    \le&\sum_{s=1}^{m-1} (2c^2s+2L^2)\eta^2 \sum_{j=1}^s \ex{\norm{v^{j-1}}^2} \\
	    &\quad- (1-L\eta)\sum_{s=0}^{m-1}\ex{\norm{v^s}^2}\\
	    \le&\sum_{s=0}^{m-1}\paren{m(m-1)c^2\eta^2 + 2L^2\eta^2(m-1)-(1-L\eta)}\ex{\norm{v^s}^2}.
    \end{align*}
    Therefore, with $0 < \eta \le \frac{2}{L\paren{1+\sqrt{1+8(m-1)+4m(m-1)c^2/L^2}}}$, we have $m(m-1)c^2\eta^2 + 2L^2\eta^2(m-1)-(1-L\eta) \le 0$ and the proof is finished.


\subsection{Proof of Lemma \ref{lem:trace_concaten}}
\label{proof:lem:trace_concaten}
 



First, we write 
\begin{align*}
& \nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s) - v^s \\
=&\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^{s-1}) - v^{s-1} \\
&\quad+ [\nabla f_k(y^s) - \nabla f_k(y^{s-1})] - [v^s - v^{s-1}].
\end{align*}
Let $\mathscr{F}_s$ denote the $\sigma$-algebra generated by all random sample selections in sub-iteration $0, \cdots, s-1$. We have
\begin{align*}
	&\ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s) - v^s}^2 \cond \mathscr{F}_s} \\
	=& \norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^{s-1}) - v^{s-1}}^2 \\
	& +  \norm{\nabla f_k(y^s) - \nabla f_k(y^{s-1})}^2   + \ex{\norm{v^s - v^{s-1}}^2 \cond \mathscr{F}_s}  \\
	& + 2\big\langle \nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^{s-1}) - v^{s-1}, \\
	& \quad\quad\quad   \nabla f_k(y^s) - \nabla f_k(y^{s-1}) \big\rangle  \\
	& -2\big\langle  \nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^{s-1}) - v^{s-1}, \\
	&\quad\quad\quad \ex{v^s - v^{s-1} \cond \mathscr{F}_s} \big\rangle  \\
	&-2 \innprod{\nabla f_k(y^s) - \nabla f_k(y^{s-1}), \ex{v^s - v^{s-1} \cond \mathscr{F}_s}} \\
	 =& \norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^{s-1}) - v^{s-1}}^2  \\
	& \quad - \norm{\nabla f_k(y^s) - \nabla f_k(y^{s-1})}^2 + \ex{\norm{v^s - v^{s-1}}^2\cond \mathscr{F}_s},
\end{align*}
where the second equality follows from
\begin{align*}
	\ex{v^s - v^{s-1} \cond \mathscr{F}_s} & = \ex{\nabla \ell_z(y^s) - \nabla \ell_z(y^{s-1}) \cond \mathscr{F}_s} \\
	& = \nabla f_k (y^s) - \nabla f_k (y^{s-1}),
\end{align*}



%	

Taking expectation over $\mathscr{F}_s$ gives
\begin{align*}
		&\ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^s) - v^s}^2} \\
		=&\ex{\norm{\nabla f(y^0) - \nabla f_k(y^0) + \nabla f_k(y^{s-1}) - v^{s-1}}^2}  \\
		& - \ex{\norm{\nabla f_k(y^s) - \nabla f_k(y^{s-1})}^2} + \ex{\norm{v^s - v^{s-1}}^2}.
	\end{align*}
Telescoping the above equality we obtain the claimed result.


 

==> proof_outline_dsvrg.tex <==
\section{Useful Lemma}
We first establish the following Lemma which will be useful in the proof of D-SVRG and D-MiG.
\begin{lemma}
\label{lem:rsp666}
When Assumption~\ref{assum:l_smooth},\ref{assum:l_convex} and one of the distributed smoothness (Assumption \ref{assum:f_restricted} or \ref{assum:f_nrestricted}) hold, we have
\begin{equation*}
\ex{\norm{\nabla \ell_z(y) - \nabla \ell_z(\tx)}^2} \le 2LD_f(\tx, y) + 
\begin{cases}
2cL\paren{\norm{\tx - x^*}^2 + \norm{y-x^*}^2} &   Assumption~\ref{assum:f_restricted} \\
2cL\norm{\tx - y}^2 &   Assumption~\ref{assum:f_nrestricted}
\end{cases}
\end{equation*}
where $z$ is randomly selected from $M_k$, where 
$	D_f(x_1, x_2) = f(x_1) - f(x_2) - \innprod{\nabla f(x_2), x_1 - x_2}$.
\end{lemma}
\begin{proof}
Given $f$ is $L$-smooth and convex, the Bregman divergence $D_f(x_1, x_2)$
 is $L$-smooth and convex as a function of $x_1$.  When Assumption \ref{assum:l_smooth} and \ref{assum:l_convex} hold, we have
\begin{align*}
0 &= D_{\ell_z}(y_2, y_2) = \min_x D_{\ell_z} (x,y_2) \\
&\le D_{\ell_z} (y_1,y_2) - \frac{1}{2L}\norm{\nabla_{y_1} D_{\ell_z} (y_1,y_2)}^2\\
&= D_{\ell_z} (y_1,y_2) - \frac{1}{2L}\norm{\nabla \ell_z(y_1) - \nabla \ell_z(y_2)}^2.
\end{align*}
Averaging the inequality over $z\in M_k$ gives
\begin{align}
2LD_{f_k}(y_1, y_2) & \ge \frac{1}{|M_k|}\sum_{z\in M_k}\norm{\nabla \ell_z(y_1) - \nabla \ell_z(y_2)}^2  \nonumber \\
& =\mathbb{E}_{z\sim \mathcal{U}(M_k)}\left[\norm{\nabla \ell_z(y_1) - \nabla \ell_z(y_2)}^2\right].
\label{equ:lem1step1}
\end{align}
Assumption \ref{assum:f_restricted} allows us to compare $D_f$ and $D_{f_k}$:
\begin{align*}
	& |D_{f_k}(\tx, y) - D_{f}(\tx, y)| \\
	= &|D_{f-f_k}(\tx, y)|\\
	 =& \Big|D_{f-f_k}(\tx, x^*) + D_{f-f_k}(x^*, y) \\
	 & \quad + \innprod{\nabla(f-f_k)(x^*) - \nabla(f-f_k)(y), \tx - x^*} \Big| \\
	 \le& \frac{c}{2}\norm{\tx - x^*}^2 + \frac{c}{2}\norm{x^* - y}^2 + c\norm{x^*-y}\norm{\tx-x^*}\\
	 \le& c\paren{\norm{\tx - x^*}^2+\norm{x^*-y}^2}.
\end{align*}
Following similar arguments, using Assumption \ref{assum:f_nrestricted} we obtain a tighter bound: $|D_{f_k}(\tx, y) - D_{f}(\tx, y)| \le c\norm{\tx - y}^2$. Combining the estimate in equation (\ref{equ:lem1step1}) proves the lemma.
\end{proof}


==> regSVRG_arxiv.tex <==
%Under i.i.d. and balanced data, this requirement can be justified for large enough data size, see Appendix~\ref{sec:discussions}. 

\section{Regularization Helps Unbalanced Data}
\label{sec:regSVRG}
 
 So far, we have established the convergence when the distributed smoothness is not too large. While it may be reasonable in certain  settings, e.g. in a data center where one has control over how to distribute data, it is increasingly harder to satisfy when the data are generated locally and heterogeneous across workers. However, when such conditions are violated, the algorithms might diverge. In this situation, adding a regularization term might ensure the convergence, at the cost of possibly slowing down the convergence rate. We consider regularizing the local gradient update of D-SVRG in Alg.~\ref{alg:dissvrg_main} as
\begin{equation}\label{eq:regularized_update}
v_k^{t,s+1}  = \nabla \ell_z(\subx_{k}^{t,s+1}) -\nabla \ell_z(\tx^{t}) + \nabla f(\tx^{t}) + \mu_k (\subx_{k}^{t,s+1} - \tx^t),
\end{equation}
where the last regularization term penalizes the proximity between the current iterates $\subx_{k}^{t,s+1}$ and the reference point $\tx^t$, where $\mu_k>0$ is the regularization parameter employed at the \sout{$k$th}{\color{red}$\tth{k}$} worker. We have the following theorem.

\begin{theorem}[Distributed Regularized SVRG (D-RSVRG)]\label{thm:rsvrg}
Suppose that Assumptions \ref{assum:l_smooth}, \ref{assum:l_convex} and \ref{assum:f_sc} hold, and Assumption~\ref{assum:f_restricted} holds with $c_k < (\sigma+\mu_k)/4$. Let $\mu = \min_{1\leq k\leq n} \mu_k$. With proper $m$ and step size $\eta$, there exists some constant $0\le \nu < 1$ such that the iterates of D-RSVRG satisfy
\begin{align} \label{eq:rate_drsvrg}
\ex{f(\tx^{t+1}) - f^*} \le& \left(1- (1-\nu)\max\left\{\frac{\sigma}{L+\mu},1-\frac{\mu}{\sigma}\right\}\right) \cdot \ex{f(\tx^t) - f^*},
\end{align}
and the runtime complexity of finding an $\epsilon$-optimal solution is bounded by
\small
\[
\mathcal{O}\paren{(N/n + 
	\zeta^{-2}\bar{\kappa})\zeta^{-1} \min\left\{\kappa + \frac{\mu}{\sigma},\frac{1}{\max\{ 1 -\mu/\sigma, 0 \} }\right\}\log(1/\epsilon)}, 
\]
\normalsize
where $\zeta = 1 - 4c/(\sigma+\mu)$ and $\bar{\kappa} = (L+\mu)/(\sigma +\mu)$.
\end{theorem}

Compared with Theorem~\ref{thm:dissvrgII}, 
Theorem~\ref{thm:rsvrg} relaxes the assumption $c_k<\sigma/4$ to $c_k<(\sigma+\mu_k)/4$, which means that by inserting a larger regularization $\mu_k$ to local workers that are not distributed smooth, i.e. those with large $c_k$, one can still guarantee the convergence of D-RSVRG. However, increasing $\mu$ leads to a slower convergence rate: a large $\mu=8L$ leads to an iteration complexity $\mathcal{O}(\kappa \log(1/\epsilon))$, similar to gradient descent.  Compared with SCOPE \cite{zhao2017scope} which requires a uniform regularization $\mu>L-\sigma$, our analysis applies tailored regularization to local workers, and potentially allows much smaller regularization to guarantee the convergence, since $c_k$'s can be much smaller than the smoothness parameter $L$.
 
